CoViT: Real-time phylogenetics for the SARS-CoV-2 pandemic using Vision Transformers

Real-time viral genome detection, taxonomic classification and phylogenetic analysis are critical for efficient tracking and control of viral pandemics such as Covid-19. However, the unprecedented and still growing amounts of viral genome data create a computational bottleneck, which effectively prevents the real-time pandemic tracking. For genomic tracing to work effectively, each new viral genome sequence must be placed in its pangenomic context. Re-inferring the full phylogeny of SARS-CoV-2, with datasets containing millions of samples, is prohibitively slow even using powerful computational resources. We are attempting to alleviate the computational bottleneck by modifying and applying Vision Transformer, a recently developed neural network model for image recognition, to taxonomic classification and placement of viral genomes, such as SARS-CoV-2. Our solution, CoViT, places SARS-CoV-2 genome accessions onto SARS-CoV-2 phylogenetic tree with the accuracy of 94.2%. Since CoViT is a classification neural network, it provides more than one likely placement. Specifically, one of the two most likely placements suggested by CoViT is correct with the probability of 97.9%. The probability of the correct placement to be found among the five most likely placements generated by CoViT is 99.8%. The placement time is 0.055s per individual genome running on NVIDIAs GeForce RTX 2080 Ti GPU. We make CoViT available to research community through GitHub: https://github.com/zuherJahshan/covit.

==> future.tex <==
CoViT is an ongoing project. We aspire to continuously enhance and improve it, mainly along the following lines:

\begin{itemize}
    \item Increase the number of lineages CoViT can classify to. Due to the limited number of the original sequenced genome in each lineage, the progress in this direction can be achieved by using augmented data (inspired by~\cite{van2001art}). We plan to create a large number of synthetic genomes per each lineage, whereas such a synthetic genome is obtained by randomly injected a limited number of edits into existing original genomes. 
    %The number of the injected edits should be such that the genome would not be accidentally transformed into another lineage.     
    \item Investigate deepening the network to further increase the accuracy of the placement.
    \item Adopt CoViT to phylogenetic analysis of other pathogens.
    \item Adopt CoViT to other healthcare related vision classification tasks such as variant calling (in human genome pipeline) and many others.  
    
\end{itemize}

%- PLOS computational biology
%- PLOS One
%- Bioinformatics 
%- BMC Bioinformatics
% https://www.sciencedirect.com/journal/computers-in-biology-and-medicine



==> results_old.tex <==
\subsubsection{Data set}
We use the COVID-19 Data Portal~\cite{covid19data} as a source of the sequenced SARS-CoV-2 genomes. 
We sort the SARS-CoV-2 lineages based on the number of sequenced genomes (accessions) in each lineage. Neural network training requires a training set of a sufficient size to provide an accurate classification result. However, only a limited number of lineages have sufficient amount of sequenced genomes (accessions), thus limiting the number of lineages CoViT is able to accurately classify a newly sequenced SARS-CoV-2 genome to. The number of lineages with at least 256 accessions reaches only 375 out of 1536 recorded lineages. Most of the lineages has less than 50 accessions available as depicted in Figure~\ref{fig:hist}.

% \begin{figure}[!t]
%   \begin{center}
%     \includegraphics[scale=0.65]{figs/hist.png}
%   \end{center}
% \caption{Accession (the number of sequenced genomes per lineage) histogram. Most of the lineages (approximately 800 out of 1536) have less than 50 accessions available. The peak in the 4000 bin accounts for all lineages with more than 3950 accessions.
% }
% \label{fig:hist}
% \end{figure}

\subsubsection{Classification groups}
We create four groups of lineages based on the number of accessions in each, as follows:
\begin{itemize}
    \item CG1: 107 lineages, with at least 2048 sequenced genomes in each. To build the dataset for this group we take from each lineage exactly 2048 samples (i.e., sequenced genomes).
    \item CG2: 189 lineages, with at least 1024 sequenced genomes in each. To build the dataset for this group we take from each lineage exactly 1024 samples.
    \item CG3: 269 lineages, with at least 512 sequenced genomes in each. To build the dataset for this group we take from each lineage at least 512 samples, and 1024 samples at most.
    \item CG4: 375 lineages, with at least 256 sequence genomes in each. To build the dataset for this group we take from each lineage at least 256 samples, and 1024 samples at most.
\end{itemize}

The purpose of this division is to investigate how much the size of the training set affects the accuracy of the placement.  

\subsubsection{Classification accuracy criterion}
CoViT classifies a newly sequenced (query) genome by sorting the known lineages in the descending order of their similarity to it. Therefore, one or two lineages of the highest similarity to the query genome are of the most interest. 

We use the top-n accuracy as CoViT placement accuracy criterion. It estimates the likelihood of the \emph{correct} result (i.e. the lineage that fits the query genome) appearing among the \emph{n} highest-probability results (i.e. \emph{n} lineages placed by the network at the top of the descending-order similarity list). Specifically, we measure the top-1, top-2 and top-5 accuracy for every classification group. %Note, the top-2 accuracy is identical to the probability of placing a sample with the correct sister node. 
Since the Covid-19 Data Portal assigns all sequenced genomes to their respective lineages, we know during the network training which results are correct, and therefore are able to tag them.     

\subsubsection{Network training}
\label{Network training}
We train CoViT for each classification group, using the following training and validation datasets:
\begin{itemize}
    \item 80\% of the sequenced genomes are applied as the training set
    \item Remaining 20\% are employed as the validation set  
\end{itemize}
We train CoViT on NVIDIA's GeForce RTX 2080 Ti GPU with an 11GB / 14Gbps GDDR6 frame buffer, running at 1.545GHz. CoViT was implemented using the TensorFlow framework in Python. To train the network, we use two main techniques, the Greedy Layer-Wise Pretraining~\cite{bengio2006greedy} and Transfer Learning~\cite{torrey2010transfer}.

\paragraph{Greedy Layer-Wise Pretraining}
Training deep neural networks is challenging due to the vanishing gradient problem (i.e. the weights in layers close to the input layer are not updated in response to errors calculated on the training dataset). The Greedy Layer-Wise Pretraining allows deep neural networks to be successfully trained, achieving state-of-the-art performance. Pretraining involves adding a new hidden layer to a model and refitting, allowing the new model to learn the inputs from the existing hidden layers, while keeping the weights for the existing hidden layers fixed and not trainable. This technique is based on the observation that training a shallow network is easier than training a deep one~\cite{bengio2006greedy}.

\paragraph{Transfer Learning}
A technique that focuses on storing knowledge gained while solving one problem, and applying it to a different but related problem~\cite{west2007spring}. In transfer learning, we first train a base network on a base dataset and task, and then we re-purpose the learned features, or transfer them, to a second target network to be trained on a target dataset and task. This works well if the features are general, meaning suitable to both base and target tasks, rather than being specific to the base task~\cite{yosinski2014transferable}.

\paragraph{Regularization}
To generalize the results on the training set better, we use several regularization techniques in parallel. We employ a dropout after each MSA and MLP sub-layers in the network. Moreover we use L2 regularization~\cite{krogh1991simple} on the trainable weights of the network (not including the biases).

\subsection{Evaluation results}
\subsubsection{Classification accuracy}
We started by building a CoViT model for the CG3 classification group. To develop deeper networks and achieve best results we chose the following hyper-parameters
\begin{center}
\begin{tabular}{||c|c|c|c|c|c|c||} 
 \hline
 $d_{model}$ & $d_{v}$ & $d_{k}$ & $d_{ff}$ & $heads$ & $dropout\_rate$ & $regularization\_coef$ \\ [0.5ex] 
 \hline\hline
 256 & 96 & 96 & 1536 & 18 & 0.1 & 0.0001 \\ [1ex]
 \hline
\end{tabular}
\end{center}
Also, we chose the $kmer$ length to be $16$, the fragment length to be $256$ (i.e., equal to the $d_{model}$) and the comperession factor, $n$, is set at $256$. These parameters are applied to all trained models.
We started training a model for the CG3 classification group using Supervised Greedy Layer-Wise Pretraining~\cite{bengio2006greedy}. We started the pretraining process by building a base model consisting of two TE layers. We trained the model for 60 epochs with a batch size of 256 \emph{examples} (i.e., assembled genomes). The average training time per epoch was 8.58[min], achieving the top-1 accuracy of 79.3\% on the validation set. Then we added two new TE layers to the base model, generating a 4-layer TE model. This 4-layer model was trained for 120 epochs, with the batch size of 256 examples. The average training time per epoch was 16.84[min]. We achieved the top-1 accuracy of 92.7\%, top-2 accuracy of 97.2\% and top-5 accuracy of 99.1\% on the validation set. The accuracy as a function of the number of epochs is depicted in Figure~\ref{fig:accs}(c).

To build the CoViT model for the CG1, CG2 and CG4 classification groups we used transfer learning~\cite{torrey2010transfer}. More specifically, we took the 4-layer learnt model for the CG3 as the base for the CG2 and the CG4 models, where the only component to change was the MLP head (presented in section~\ref{transformers}). We then trained each model for a number of epochs specified in Table~\ref{Tab:t1}, with a batch size of 256 examples. 

The accuracy as a function of the number of epochs for these remaining classification groups is presented in Figure~\ref{fig:accs}(a), (b) and (d).
Following are the validation set results. The model for CG1 classification group achieves the highest top-1 accuracy of 97.1\%, top-2 accuracy of 99.0\% and top-5 accuracy of 99.8\%. Respectively, the model for CG2 classification group achieves the highest top-1 accuracy of 95.8\%, top-2 accuracy of 98.1\% and top-5 accuracy of 99.8\%.
The model for CG3 classification group achieves the highest top-1 accuracy of 92.7\%, top-2 accuracy of 97.2\% and top-5 accuracy of 99.1\%. The model for CG4 classification group achieves the highest top-1 accuracy of 92.1\%, top-2 accuracy of 96.9\% and top-5 accuracy of 99.1\%.
These accuracy results and additional training information are summarized in Table~\ref{Tab:t1}. 

\begin{figure}[!t]
  \begin{center}
    \includegraphics[scale=0.43]{figs/Accuracy_fig6.png}
  \end{center}
\caption{Accuracy vs. number of epochs for different models and four classification groups: CG1 (a), CG2 (b), CG3 (c) and CG4 (d). 
%The model for 107Lins classification group achieves highest top-1 accuracy on validation set of 97.1\%, top-2 accuracy of 99.0\% and top-5 accuracy of 99.8\%. The model for 189Lins classification group achieves highest top-1 accuracy on validation set of 95.8\%, top-2 accuracy of 98.1\% and top-5 accuracy of 99.8\%.
%The model for 269Lins classification group achieves highest top-1 accuracy on validation set of 92.7\%, top-2 accuracy of 97.2\% and top-5 accuracy of 99.1\%. The model for 375Lins classification group achieves highest top-1 accuracy on validation set of 92.1\%, top-2 accuracy of 96.9\% and top-5 accuracy of 99.1\%.
}
\label{fig:accs}
\end{figure}

\begin{table}[ht]
\caption{Accuracy results and training information of the different models on the different classification groups\label{Tab:t1}}
\begin{center}
\begin{tabular}{||c|c|c|c|c|c|c||}
\hline
classification group & transferred from & epochs & avg $\frac{train\_time}{epoch}$ & top-1 acc & top-2 acc & top-5 acc\\ [0.5ex] 
\hline\hline
CG1 & CG2 & 15 & 12.89min & 97.1\% & 99.0\% & 99.8\% \\
\hline
CG2 & CG3 & 40 & 13.09min & 95.8\% & 98.1\% & 99.8\% \\
\hline
CG3 & - & 60, 120 & 8.58min, 16.84min & 92.7\% & 97.2\% & 99.1\% \\
\hline
CG4 & CG3 & 155 & 21.52min & 92.1\% & 96.9\% & 99.1\% \\ [1ex]
\hline
\end{tabular}
\end{center}
\end{table}
%Results of the accuracy achieved at each epoch are depicted in Figure~\ref{fig:accs}.


\subsubsection{Training and inference times}
The following Table~\ref{Tab:t2} summarizes the training and inference times for each classification group. Inference time for the CG1 is 1.45[ms] which is almost three orders of magnitude faster than probably the fastest state of the art placement tool UShER~\cite{turakhia2021ultrafast}.

\begin{table}[ht]
\caption{Training and inference time of the various models.\label{Tab:t2}}
\begin{center}
\begin{tabular}{||c|c|c||} 
 \hline
 classification group & train time per example & inference time per example\\ [0.5ex] 
 \hline\hline
 CG1 & 4.59ms & 1.45ms\\
 \hline
 CG2 & 4.67ms & 1.47ms\\
 \hline
 CG3 & 4.70ms & 1.49ms\\
 \hline
 CG4 & 4.71ms & 1.49ms\\ [1ex]
 \hline
\end{tabular}
\end{center}
\end{table}

\subsubsection{Comparison with state-of-the-art}
Several methods have been developed for the purpose of placing genome sequence samples onto an existing reference phylogeny tree~\cite{minh2020iq, barbera2019epa, loytynoja2012accurate, ruan2007treefam}. However, these methods are far too slow to enable real-time genomic placement.
To address the speed of interpretation of viral transmission and evolutionary dynamics, ultrafast bootstrapping~\cite{hoang2018ufboot2, minh2013ultrafast} have been recently developed. While those methods provide significant speedup, they are not applicable to the problem of placing individual samples onto a reference phylogeny. 

Below we address several state of the art classification and placement tools, including Kraken~\cite{wood2019improved}, PACIFIC~\cite{acera2021pacific}, UShER~\cite{turakhia2021ultrafast} and PangoLearn~\cite{o2021assignment}.
%\begin{itemize}
%    \item Kraken
%    \item PACIFIC
%    \item UShER
 %   \item PangoLearn
%\end{itemize}

%We focus our comparison on state of the art virus classifier, i.e. UShER and PangoLearn?.

Kraken is one of the most popular genome classifiers. It uses exact matching of kmers of the genome(s) in question against a known organisms' genomes database. Kraken was not specifically designed to classify SARS-CoV-2 (or another viral pathogen with pandemic potential) lineages and therefore is not sensitive enough to place SARS-CoV-2 variants which differ from one another by only several basepairs. 

PACIFIC is arguably the first deep classification neural network based genome classifier. PACIFIC has been shown to classify genomes into a very limited group of classes (5 distinct virus classes and a human genome class).    

%UShER is one of the latest phylogenetic placement tools. 
%UShER uses a maximum parsimony approach where it searches the entire reference variant-annotated tree %(Fig. 1 and Methods) 
%for a placement that requires the fewest additional mutations. It is capable of classifying a SARS-CoV-2 genome into the correct sister 
%node with an accuracy of 97.2\%. UShER takes approximately 0.5[s] to place 
%a single sample onto the SARS-CoV-2 phylogenetic tree, and approximately 18[s] to place 1,000 samples. One notable limitation of UShER is that it only supports mutations caused by replacements (does not support mutations caused by indels).

PangoLearn is an algorithm for lineage assignment which relies on machine learning and uses random forests. The model was trained using SARS-CoV-2 sequences from GISAID~\cite{gisaid}.

\begin{figure}[!t]
  \begin{center}
    \includegraphics[scale=0.25]{figs/covitvsusher.png}
  \end{center}
\caption{CoViT accuracy of the different models against UShER on a randomly selected set of accessions. 
}
\label{fig:cvu}
\end{figure}

We compare the top-1 accuracy and placement speed of four CoViT models  (i.e., CG1, CG2, CG3, CG4) against UShER~\cite{turakhia2021ultrafast} by placing 13,500 genome assemblies randomly selected from the Covid-19 Data Portal~\cite{covid19data}. 
UShER is one of the latest phylogenetic placement tools. It uses a maximum parsimony approach where it searches the entire reference variant-annotated tree %(Fig. 1 and Methods) 
for a placement that requires the fewest additional mutations. 
%It is capable of classifying a SARS-CoV-2 genome into the correct sister node with an accuracy of 97.2\%. UShER takes approximately 0.5[s] to place a single sample onto the SARS-CoV-2 phylogenetic tree, and approximately 18[s] to place 1,000 samples. 
One reported limitation of UShER is that it only supports mutations caused by replacements (does not support mutations caused by indels).

For models CG1 through CG4, CoViT achieves the average placement accuracy of 96.1\%, 94.2\%, 93.8\% 93.9\% respectively, while UshER's average accuracy is 92.1\% as depicted in Figure~\ref{fig:cvu}. To test the placement speed, we ran both CoViT and UShER on Intel i7-9700K CPU with 8 cores, operating at 3.60GHz. Additionally, CoViT was implemented on NVIDIA’s GeForce RTX
2080 Ti GPU. The placement times for these 13,500 genome assemblies are presented in table~\ref{Tab:t3}. The rest of the table is adopted from \cite{turakhia2021ultrafast}.

% TODO: What should I write in order to append the table from the UShER paper as well. Maybe: "Although we did not compare CoViT with other phylogeny placement tools, according to table XX, taken from ~\cite{UshER}" it is clear that CoViT achieves state-of-the-art performance."

\begin{table}[t]
\caption{Placement time of 13,500 SARS-CoV-2 genomes assemblies. 
%The results of placement algorithms other than  CoViT and UShER are adopted from~\cite{turakhia2021ultrafast}.
\label{Tab:t3}}
\begin{center}
\begin{tabular}{||c|c|c||} 
 \hline
 program & time & speedup vs UshER\\ [0.5ex]
 \hline\hline
 CG1 (GPU) & 12.42m & 3.6\\
 \hline
 CG2 (GPU) & 12.45m & 3.6\\
 \hline
 CG3 (GPU) & 12.47m & 3.6\\
 \hline
 CG4 (GPU) & 12.52m & 3.5\\
 \hline
 CG1 (CPU) & 21.35m & 2.1\\
 \hline
 CG2 (CPU) & 21.35m & 2.1\\
 \hline
 CG3 (CPU) & 21.35m & 2.1\\
 \hline
 CG4 (CPU) & 21.38m & 2.1\\
 \hline
 UshER & 44.1m & 1\\ [1ex]
 \hline
\end{tabular}
\end{center}
\end{table}
